Costello's pushforward formula: errata and generalization

K. Costello's Pushforward Formula is not correct as stated. We verify it holds under an assumption of properness or of a weaker notion we call "purity." We then check many papers that used this formula to make sure it holds in their context.

==> abstract.tex <==
K. Costello's Pushforward Formula \cite[Theorem 5.0.1]{Costello} is not correct as stated. We verify it holds under an assumption of properness or of a weaker notion we call ``purity.'' We then check many papers that used this formula to make sure it holds in their context. 
